LoRA-Squeeze: Simple and Effective Post-Tuning and In-Tuning Compression of LoRA Modules

Despite its huge number of variants, standard Low-Rank Adaptation (LoRA) is still a dominant technique for parameter-efficient fine-tuning (PEFT). Nonetheless, it faces persistent challenges, including the pre-selection of an optimal rank and rank-specific hyper-parameters, as well as the deployment complexity of heterogeneous-rank modules and more sophisticated LoRA derivatives. In this work, we introduce LoRA-Squeeze, a simple and efficient methodology that aims to improve standard LoRA learning by changing LoRA module ranks either post-hoc or dynamically during training}. Our approach posits that it is better to first learn an expressive, higher-rank solution and then compress it, rather than learning a constrained, low-rank solution directly. The method involves fine-tuning with a deliberately high(er) source rank, reconstructing or efficiently approximating the reconstruction of the full weight update matrix, and then using Randomized Singular Value Decomposition (RSVD) to create a new, compressed LoRA module at a lower target rank. Extensive experiments across 13 text and 10 vision-language tasks show that post-hoc compression often produces lower-rank adapters that outperform those trained directly at the target rank, especially if a small number of fine-tuning steps at the target rank is allowed. Moreover, a gradual, in-tuning rank annealing variant of LoRA-Squeeze consistently achieves the best LoRA size-performance trade-off.

==> sections/06_conclusion_icml.tex <==
%\section{Conclusion and Future Work}
\section{Conclusion}
We introduced {\em \method}, a simple yet effective methodology for compressing LoRA modules either post-hoc or dynamically during fine-tuning. Our experiments over a suite of 13 text-based and 10 vision-language VQA tasks demonstrated that it is often more advantageous to fine-tune with a higher, `overparameterized' LoRA rank and then compress to a lower target rank, rather than fine-tuning at the fixed target rank directly. This approach not only yields modules with a better size-to-performance trade-off but also simplifies deployment by decoupling the training rank from the deployment rank and reducing the need for rank-specific hyperparameter tuning. %The gradual, in-tuning rank annealing variant delivered the most robust results in general.

One future research direction is extending the \method principles to more sophisticated LoRA variants.

%Due to its wide adoption, extensive use and architectural simplicity, in this work we focused on the standard LoRA design. For future work, one research direction is to extend the LoRA-Squeeze principles beyond standard LoRA setups to more sophisticated LoRA variants. We also plan to utilize \method principles in techniques for module merging~\citep{stoica2025iclr}. Furthermore, we plan to explore methods for automatically determining the optimal source rank or gradual rank annealing schedules for a given target rank by extending our preliminary analyses (see Figure~\ref{fig:ret_tasks} in the Appendix) on the rate of decay of singular values during decomposition. 
